S-Walk: Accurate and Scalable Session-based Recommendationwith Random Walks

Session-based recommendation (SR) predicts the next items from a sequence of previous items consumed by an anonymous user. Most existing SR models focus only on modeling intra-session characteristics but pay less attention to inter-session relationships of items, which has the potential to improve accuracy. Another critical aspect of recommender systems is computational efficiency and scalability, considering practical feasibility in commercial applications. To account for both accuracy and scalability, we propose a novel session-based recommendation with a random walk, namely S-Walk. Precisely, S-Walk effectively captures intra- and inter-session correlations by handling high-order relationships among items using random walks with restart (RWR). By adopting linear models with closed-form solutions for transition and teleportation matrices that constitute RWR, S-Walk is highly efficient and scalable. Extensive experiments demonstrate that S-Walk achieves comparable or state-of-the-art performance in various metrics on four benchmark datasets. Moreover, the model learned by S-Walk can be highly compressed without sacrificing accuracy, conducting two or more orders of magnitude faster inference than existing DNN-based models, making it suitable for large-scale commercial systems.

==> Figures/Fig9_session_length_ours.tex <==
\begin{figure}
\centering

\begin{tabular}{c}
\includegraphics[width=0.440\textwidth]{Figures/Fig9_cropped_legend.pdf}
\end{tabular}


\begin{tabular}{cc}
\includegraphics[width=0.220\textwidth]{Figures/Fig9_appendix_DIGI5_Recall.pdf} &
\includegraphics[width=0.220\textwidth]{Figures/Fig9_appendix_DIGI5_MAP.pdf} \\
\end{tabular}
(a) DIGI5 \\

\begin{tabular}{cc}
\includegraphics[width=0.220\textwidth]{Figures/Fig9_appendix_RR_Recall.pdf} &
\includegraphics[width=0.220\textwidth]{Figures/Fig9_appendix_RR_MAP.pdf} \\
%(a) RR & (a) DIGI5  \\
\end{tabular}
(b) RR  \\



\vskip -0.1in
\caption{R@20 and MAP@20 of our proposed models over different session lengths on DIGI5 and RR. Let $\mathbf{Tran}$ and $\mathbf{Tele}$ denote our transition model and teleportation model, respectively.}
\label{fig:length_proposed}
\vskip -0.2in
\end{figure}




% \begin{figure}
% \centering
% \begin{tabular}{cc}
% \includegraphics[width=0.220\textwidth]{Figures/Fig4_RR_Recall.pdf} &
% \includegraphics[width=0.220\textwidth]{Figures/Fig4_RR_MAP.pdf} \\
% \end{tabular}
% (a) RR  \\
% \begin{tabular}{cc}
% \includegraphics[width=0.220\textwidth]{Figures/Fig4_DIGI5_Recall.pdf} &
% \includegraphics[width=0.220\textwidth]{Figures/Fig4_DIGI5_MAP.pdf} \\
% \end{tabular}
% (b) DIGI5  \\
% \vskip -0.1in
% \caption{R@20 and MAP@20 of S-Walk and state-of-the-art models with different session lengths (Short $\le$ 5, Long > 5) on two benchmark datasets.}
% \label{fig:length_baseline}
% \vskip -0.15in
% \end{figure}

